Made-to measure galaxy models - I Methodology

We re-derive the made-to-measure method of Syer and Tremaine 1996, for modelling stellar systems and individual galaxies, and demonstrate how extensions to the made-to-measure method may be implemented and used. We illustrate the enhanced made-to-measure method by determining the mass-to-light ratio of a galaxy modelled as a Plummer sphere. From the standard galactic observables of surface brightness and line-of-sight velocity dispersion together with the h_4 Gauss-Hermite coefficient of the line-of-sight velocity distribution, we successfully recover the true mass-to-light ratio of our toy galaxy. Using kinematic data from Kleyna et al 2002, we then estimate the mass-to-light ratio of the dwarf spheroidal galaxy Draco achieving a V-band value of 539 \pm 136 M_{\odot} / L_{\odot}. We describe the main aspects of creating a made-to-measure galaxy model and show how the key modelling parameters may be determined.

==> abstract <==
We re-derive the made-to-measure method of Syer and Tremaine 1996, for modelling stellar systems
and individual galaxies, and demonstrate how extensions to the made-to-measure method may be 
implemented and used.  We illustrate the enhanced made-to-measure method by determining the 
mass-to-light ratio of a galaxy modelled as a Plummer sphere.   From the standard galactic 
observables of surface brightness and line-of-sight velocity dispersion together with 
the $h_4$ Gauss-Hermite coefficient of the line-of-sight velocity distribution,  we successfully 
recover the true mass-to-light ratio of our toy galaxy.  Using kinematic data from Kleyna et al 2002,
we then estimate the mass-to-light ratio of the dwarf spheroidal galaxy Draco achieving a V-band 
value of 539 \pm 136 M_{\odot} / L_{\odot}.  We describe the main aspects of creating 
a made-to-measure galaxy model and show how the key modelling parameters may be determined.

